TeleAware Robot: Designing Awareness-augmented Telepresence Robot for Remote Collaborative Locomotion

Telepresence robots can be used to support users to navigate an environment remotely and share the visiting experience with their social partners. Although such systems allow users to see and hear the remote environment and communicate with their partners via live video feed, this does not provide enough awareness of the environment and their remote partner's activities. In this paper, we introduce an awareness framework for collaborative locomotion in scenarios of onsite and remote users visiting a place together. From an observational study of small groups of people visiting exhibitions, we derived four design goals for enhancing the environmental and social awareness between social partners, and developed a set of awareness-enhancing techniques to add to a standard telepresence robot - named TeleAware robot. Through a controlled experiment simulating a guided exhibition visiting task, TeleAware robot showed the ability to lower the workload, facilitate closer social proximity, and improve mutual awareness and social presence compared with the standard one. We discuss the impact of mobility and roles of local and remote users, and provide insights for the future design of awareness-enhancing telepresence robot systems that facilitate collaborative locomotion.

==> bib2bbl.tex <==
\begin{document}
    \nocite{*}
    \bibliography{main.bib} %.bib文件名字
    \bibliographystyle{ACM-Reference-Format} %.bst模板
\end{document}

==> table2.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
          & Behavior Category & Subcategories & Group 1  & ~ & ~ & Group 2  & ~ & ~ & Group 3  & ~ & ~ & Group 4  & ~ & ~ & Group 5 （Effective Duration 6min ） & ~ & ~ & Group 6 （Effective Duration 1min ） & ~ & ~ & Group 7  & ~ & ~ & Group 8  & ~ & ~ & Group 9  & ~ & ~ & Group 10  & ~ & ~ & Group 11  & ~ & ~ & Group 12  & ~ & ~ & Group 13  & ~ & ~ & Group 14  & ~ & ~ & Group 15  & ~ & ~ & Group 16  & ~ & ~ & ~ \\ \hline
        Vistor Flow & ~ & ~ & Sparse & ~ & ~ & Sparse & ~ & ~ & Sparse & ~ & ~ & Sparse & ~ & ~ & Sparse & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & Crowded & ~ & ~ & ~ \\ \hline
        Participant & ~ & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & P1 & P2 & ~ & ~ \\ \hline
        Gender（Age） & ~ & ~ & Female（23） & Female（23） & ~ & Female（23） & Female（24） & ~ & Female（23） & Female（23） & ~ & Male（23） & Female（23） & ~ & Male（20） & Male（20） & ~ & Male（20） & Male（20） & ~ & Female（25） & Male（25） & ~ & Female（27） & Male（26） & ~ & Male（33） & Female（34） & ~ & Male（39） & Male（16） & ~ & Male（39） & Male（65） & ~ & Male（26） & Male（26） & ~ & Male（27） & Female（25） & ~ & Female（22） & Female（21） & ~ & Female（26） & Female（26） & ~ & Female（49） & Female（45） & ~ & ~ \\ \hline
        Leadership & ~ & ~ & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & Leader & Leader & Unable to determine leadership & ~ \\ \hline
        Duration as a Leader & ~ & ~ & 3min 48sec & 6min 24sec & 0 & 10min  & 0min  & 0min  & 3min 4sec & 6min 50sec & 14sec & 3min 57sec & 3min 50sec & 133sec & 3min 40sec & 44sec & 96sec & 0 & 0 & 1min  & 9min 39sec & 0 & 20sec & 9min 8sec & 40sec & 12sec & 4min 5sec & 4min 45sec & 70sec & 10min  & 0 & 0 & 8min 51sec & 33sec & 1min 18sec & 4min 20sec & 4min 25sec & 1min 15sec & 5min 25sec & 2min 51sec & 1min 44sec & 1min 30sec & 8min 30sec & 0 & 2min 23sec & 3min 9sec & 4min 28sec & 6min 56sec & 1min 40sec & 2min 15sec & ~ \\ \hline
        User-Environment & Visual Perception & Viewer scans the environment. & P1 59sec P2 59sec & ~ & ~ & P1 1min 34sec P2 1min 34sec & ~ & ~ & P1 55sec P2 1min 9sec & ~ & ~ & P1 2min 2sec P2 2min 2sec & ~ & ~ & P1 26sec  P2 26sec & ~ & ~ & Insufficient Duration & ~ & ~ & P1 2min 45sec P2 2min 30sec & ~ & ~ & P1 2min 27sec P2 2min 27sec & ~ & ~ & P1 37sec  P2 28sec & ~ & ~ & P1 3min 30sec P2 3min 30sec & ~ & ~ & P1 36sec P2 45sec & ~ & ~ & P1 56sec  P2 56sec & ~ & ~ & P1 41sec  P2 49sec & ~ & ~ & P1 1min 51sec P2 5min 50sec & ~ & ~ & P1 38sec  P2 1min 3sec & ~ & ~ & P1 2min  P2 2min  & ~ & ~ & ~ \\ \hline
        ~ & ~ & Viewer looks at exhibits or other people . & P1 8min 46sec P2 8min 46sec & ~ & ~ & P1 6min 17sec P2 6min 17sec & ~ & ~ & P1 8min 15sec P2 8min 1sec & ~ & ~ & P1 6min 30sec P2 6min 30sec & ~ & ~ & P1 5min 34sec  P2 5min 34sec & ~ & ~ & Insufficient Duration & ~ & ~ & P1 6min 44sec P2 7min 58sec & ~ & ~ & P1 7min 40sec P2 7min 40sec & ~ & ~ & P1 8min 52sec P2 8min 50sec & ~ & ~ & P1 5min 30sec P2 5min 30sec & ~ & ~ & P1 6min 37sec P2 6min 30sec & ~ & ~ & P1 9min 4sec  P2 9min 4sec & ~ & ~ & P1 8min 46sec  P2 8min 10sec & ~ & ~ & P1 6min 43sec  P2 3min 12sec & ~ & ~ & P1 5min 27sec P2 8min 31sec & ~ & ~ & P1 4min 26sec  P2 4min 26sec & ~ & ~ & ~ \\ \hline
        ~ & Auditory Perception & ~ & 1Instance of being distracted by sudden environmental noise. & ~ & ~ & 1Instance of being distracted by sudden environmental noise. & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 1 Instance of being distracted by exhibit video sound & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 1 Instance of being distracted by exhibit video sound & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 1 Instance of being distracted by exhibit video sound & ~ & ~ & 0 & ~ & ~ & 1 Instance of being distracted by exhibit video sound & ~ & ~ & ~ \\ \hline
        ~ & Communication with Others in The Environment & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 1 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & ~ \\ \hline
        User-Partner & Visual Perception & Viewer’s gaze is directed towards the partner. & "P1 looks at the partner:3 \\ \hline
        P2 looks at the partner:2" & "P1 looks at the partner:2 \\ \hline
        P2 looks at the partner:7" & 0 & "P1 looks at the partner:20 \\ \hline
        P2 looks at the partner:28" & 0 & 0 & "P1 looks at the partner:6 \\ \hline
        P2 looks at the partner:2" & "P1 looks at the partner:11 \\ \hline
        P2 looks at the partner:8" & 2 & "P1 looks at the partner:5 \\ \hline
        P2 looks at the partner:2" & "P1 looks at the partner:2 \\ \hline
        P2 looks at the partner:2" & 4 & "P1 looks at the partner:1 \\ \hline
        P2 looks at the partner:2" & P1 looks at the partner:1 & 1 & 0 & 0 & 1 & "P1 looks at the partner:10 \\ \hline
        P2 looks at the partner:3" & 0 & 0 & "P1 looks at the partner:8 \\ \hline
        P2 looks at the partner:5" & P1 looks at the partner:1 & 0 & P1 looks at the partner:3 P2 looks at the partner:1 & P1 looks at the partner:3 P2 looks at the partner:4 & 2 & P1 looks at the partner:12  P2 looks at the partner:6 & 0 & 0 & "P1 looks at the partner:16 \\ \hline
        P2 looks at the partner:1" & P1 looks at the partner:1 & P2 looks at the partner:1 & P2 looks at the partner:3 & "P1 looks at the partner:2 \\ \hline
        P2 looks at the partner:5" & 0 & "P1 looks at the partner:0 \\ \hline
        P2 looks at the partner:1" & "P1 looks at the partner:1 \\ \hline
        P2 looks at the partner:2" & 0 & "P1 looks at the partner:2 \\ \hline
        P2 looks at the partner:1" & "P1 looks at the partner:2 \\ \hline
        P2 looks at the partner:4" & 0 & 0 & "P1 looks at the partner:3 \\ \hline
        P2 looks at the partner:1" & 1 & "P1 looks at the partner:3 \\ \hline
        P2 looks at the partner:1" & P2 looks at the partner:1 & 2 & ~ \\ \hline
        ~ & ~ & Viewer searches for the partner with their gaze. & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 5 & 0 & 0 & 0 & 0 & 0 & 0 & P1 searches for the partner:1 & 0 & 0 & P2 searches for the partner:1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & P1 searches for the partner:2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & P1 searches for the partner:1 & 1 & 0 & 0 & 0 & "P1 searches for the partner:3 \\ \hline
        P2 searches for the partner:1" & P1 searches for the partner:1 & 1 & ~ \\ \hline
        ~ & Verbal Communication & ~ & 14 & ~ & ~ & 16 & ~ & ~ & 17 & ~ & ~ & 10 & ~ & ~ & 3 & ~ & ~ & 1 & ~ & ~ & 9 & ~ & ~ & 12 & ~ & ~ & 11 & ~ & ~ & 5 & ~ & ~ & 13 & ~ & ~ & 9 & ~ & ~ & 10 & ~ & ~ & 11 & ~ & ~ & 7 & ~ & ~ & 12 & ~ & ~ & ~ \\ \hline
        ~ & Physical Contact & Viewer touches the companion's shoulder or arm(times). & 0 & 0 & 0 & P1 touches partner's shoulder or arm with hand:1 & 0 & 0 & "P1 touches partner's shoulder or arm with hand:1 \\ \hline
        P2 touches partner's shoulder or arm with hand:1" & P2 touches partner's shoulder or arm with hand:1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & P1 touches partner's shoulder or arm with hand:1  P2 touches partner's shoulder or arm with hand:1 & 0 & 1 & 0 & 0 & 0 & P1 touches partner's shoulder or arm with hand:8  P2 touches partner's shoulder or arm with hand:1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & P1 touches partner's shoulder or arm with hand:1 & 0 & 1 & P1 touches partner's shoulder or arm with hand:1 & P1 touches partner's shoulder or arm with hand:2 & 1 & P2 touches partner's shoulder or arm with hand:2 & 0 & 0 & ~ \\ \hline
        ~ & ~ & Viewer and companion walk arm-in-arm(times). & 0 & ~ & ~ & 0 & ~ & ~ & 3 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 1 & ~ & ~ & 4 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 6 & ~ & ~ & 5 & ~ & ~ & ~ \\ \hline
        ~ & ~ & Viewer and companion hold hands(times). & 0 & ~ & ~ & 0 & ~ & ~ & 2 & ~ & ~ & 1 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & ~ \\ \hline
        ~ & Waving Gesture & ~ & 0 & ~ & ~ & 0 & ~ & ~ & ~ & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 1 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & 0 & ~ & ~ & ~ \\ \hline
        User-(Partner-Environment) & Eye Tracking & ~ & "P1 follows P2's gaze:8 \\ \hline
        P2 follows P1's gaze:6" & "P1 follows P2's gaze:19 \\ \hline
        P2 follows P1's gaze:6" & 0 & "P1 follows P2's gaze:3 \\ \hline
        P2 follows P1's gaze:7" & 0 & 0 & "P1 follows P2's gaze:4 \\ \hline
        P2 follows P1's gaze:8" & "P1 follows P2's gaze:7 \\ \hline
        P2 follows P1's gaze:3" & 0 & "P1 follows P2's gaze:5 \\ \hline
        P2 follows P1's gaze:2" & "P1 follows P2's gaze:5 \\ \hline
        P2 follows P1's gaze:1" & 5 & P2 follows P1's gaze:1 & "P1 follows P2's gaze:2 \\ \hline
        P2 follows P1's gaze:0" & 0 & 0 & 0 & 1 & "P1 follows P2's gaze:0 \\ \hline
        P2 follows P1's gaze:11" & 0 & 0 & "P1 follows P2's gaze:1 \\ \hline
        P2 follows P1's gaze:20" & P1 follows P2's gaze:3 & 1 & "P1 follows P2's gaze:1 \\ \hline
        P2 follows P1's gaze:2" & "P1 follows P2's gaze:8 \\ \hline
        P2 follows P1's gaze:2" & 1 & P1 follows P2's gaze:1  P2 follows P1's gaze:12 & 0 & 0 & "P1 follows P2's gaze:2 \\ \hline
        P2 follows P1's gaze:6" & "P1 follows P2's gaze:1 \\ \hline
        P2 follows P1's gaze:1" & 0 & "P1 follows P2's gaze:0 \\ \hline
        P2 follows P1's gaze:1" & P1 follows P2's gaze:5 & 0 & "P1 follows P2's gaze:1 \\ \hline
        P2 follows P1's gaze:3" & "P1 follows P2's gaze:7 \\ \hline
        P2 follows P1's gaze:2" & 0 & "P1 follows P2's gaze:2 \\ \hline
        " & "P1 follows P2's gaze:2 \\ \hline
        P2 follows P1's gaze:2" & 0 & "P1 follows P2's gaze:3 \\ \hline
        P2 follows P1's gaze:1" & P1 follows P2's gaze:2 & 0 & "P1 follows P2's gaze:3 \\ \hline
        P2 follows P1's gaze:14" & P1 follows P2's gaze:4 & P1 follows P2's gaze:1 & ~ \\ \hline
        ~ & Gestural Reference & ~ & "P1's gestural reference:10 \\ \hline
        P2's gestural reference:8" & "P1's gestural reference:22 \\ \hline
        P2's gestural reference:12" & 0 & "P1's gestural reference:23 \\ \hline
        P2's gestural reference:4" & 0 & 0 & "P1's gestural reference:15 \\ \hline
        P2's gestural reference:15" & "P1's gestural reference:18 \\ \hline
        P2's gestural reference:9" & 1 & "P1's gestural reference:2 \\ \hline
        P2's gestural reference:5" & "P1's gestural reference:4 \\ \hline
        P2's gestural reference:7" & 9 & 0 & 0 & 0 & 0 & 0 & 0 & "P1's gestural reference:20 \\ \hline
        P2's gestural reference:4" & 0 & 0 & "P1's gestural reference:20 \\ \hline
        P2's gestural reference:7" & "P1's gestural reference:1 \\ \hline
        P2's gestural reference:1" & 0 & "P1's gestural reference:6 \\ \hline
        P2's gestural reference:1" & "P1's gestural reference:4 \\ \hline
        P2's gestural reference:11" & 0 & P1's gestural reference:9  P2's gestural reference:2 & 0 & 0 & "P1's gestural reference:26 \\ \hline
        P2's gestural reference:6" & "P1's gestural reference:3 \\ \hline
        P2's gestural reference:1" & 0 & "P1's gestural reference:3 \\ \hline
        P2's gestural reference:2" & "P1's gestural reference:5 \\ \hline
        P2's gestural reference:2" & 3 & "P1's gestural reference:5 \\ \hline
        P2's gestural reference:4" & "P1's gestural reference:1 \\ \hline
        P2's gestural reference:5" & 2 & "P1's gestural reference:4 \\ \hline
        P2's gestural reference:2" & "P1's gestural reference:1 \\ \hline
        P2's gestural reference:2" & 3 & P1's gestural reference:1 & "P1's gestural reference:4 \\ \hline
        P2's gestural reference:2" & 0 & "P1's gestural reference:19 \\ \hline
        P2's gestural reference:3" & "P1's gestural reference:2 \\ \hline
        P2's gestural reference:4" & "P1's gestural reference:1 \\ \hline
        P2's gestural reference:1" & ~ \\ \hline
        ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
    \end{tabular}
\end{table}

==> table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{The video coding codebook based on the "User-Partner-Environment" framework.}
\begin{tabular}{lllll}
\hline
\textbf{Relationship}                                                             & \textbf{\begin{tabular}[c]{@{}l@{}}Behavior\\ Code\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Behavior\\ Category\end{tabular}}                         & \textbf{Operational Definition}                                                                                                                                                           & \textbf{Subcategories}                                                                                           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}user-\\ environment\end{tabular}}              & \multirow{2}{*}{ES}                                              & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ Perception\end{tabular}}                 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Viewers observe\\ information\\ in the environment.\end{tabular}}                                                                              & \begin{tabular}[c]{@{}l@{}}ES1: Viewer scans\\ the environment\\ (no specific target).\end{tabular}              \\ \cline{5-5} 
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}ES2: Viewer looks at\\ exhibits or \\ other people \\ (specific target).\end{tabular} \\ \cline{2-5} 
\textbf{}                                                                         & AP                                                               & \begin{tabular}[c]{@{}l@{}}Auditory\\ Perception\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Viewers pay attention\\ to other sounds\\ in the environment.\end{tabular}                                                                                     &                                                                                                                  \\ \cline{2-5} 
\textbf{}                                                                         & CO                                                               & \begin{tabular}[c]{@{}l@{}}Communication \\ with Others\\ in the \\ Environment\end{tabular} & \begin{tabular}[c]{@{}l@{}}Verbal communication\\ with people \\ other than the companion \\ in the environment.\end{tabular}                                                             &                                                                                                                  \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}user-\\ partner\end{tabular}}                  & \multirow{2}{*}{VS}                                              & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Visual\\ Perception\end{tabular}}                 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The viewer's gaze is \\ directed towards \\ or searching for\\ the partner.\end{tabular}}                                                      & \begin{tabular}[c]{@{}l@{}}VS1: directly\\ towards the partner.\end{tabular}                                     \\ \cline{5-5} 
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}VS2: search\\ for the partner.\end{tabular}                                           \\
                                                                                  &                                                                  &                                                                                              &                                                                                                                                                                                           &                                                                                                                  \\ \cline{2-5} 
\textbf{}                                                                         & VC                                                               & \begin{tabular}[c]{@{}l@{}}Verbal\\ Communication\end{tabular}                               & \begin{tabular}[c]{@{}l@{}}Viewers engage in verbal\\ communication\\ with their partner.\end{tabular}                                                                                    &                                                                                                                  \\ \cline{2-5} 
\textbf{}                                                                         & \multirow{3}{*}{PC}                                              & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Physical\\ Contact\end{tabular}}                  & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Physical contact occurs\\ between the viewer\\ and the partner.\end{tabular}}                                                                  & \begin{tabular}[c]{@{}l@{}}PC1: touch\\ shoulder or arm.\end{tabular}                                            \\ \cline{5-5} 
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           & PC2: walk arm-in-arm.                                                                                            \\ \cline{5-5} 
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           & PC3: hold hands.                                                                                                 \\ \cline{2-5} 
\textbf{}                                                                         & \multirow{2}{*}{WG}                                              & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Waving\\ Gesture\end{tabular}}                    & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Viewer waves to\\ the companion.\end{tabular}}                                                                                                 & \multirow{2}{*}{}                                                                                                \\
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           &                                                                                                                  \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}user-\\ (partner\\ -environment)\end{tabular}} & ET                                                               & \begin{tabular}[c]{@{}l@{}}Eye\\ Tracking\end{tabular}                                       & \begin{tabular}[c]{@{}l@{}}One viewer looks at \\ an exhibit, and the \\ other pne follows to \\ the same exhibit.\end{tabular}                                                           &                                                                                                                  \\ \cline{2-5} 
\textbf{}                                                                         & GR                                                               & \begin{tabular}[c]{@{}l@{}}Gestural\\ Reference\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}Viewer uses gestures\\ to refer to\\ the environment\\ or exhibits.\end{tabular}                                                                               &                                                                                                                  \\ \cline{2-5} 
\textbf{}                                                                         & \multirow{6}{*}{DO}                                              & \multirow{6}{*}{Leadership}                                                                  & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Two viewers act as\\ the leader or follower, \\ with the follower\\ moving and communicating\\ in accordance \\ with the leader.\end{tabular}} & DOP1:P1 has leadership.                                                                                          \\
                                                                                  &                                                                  &                                                                                              &                                                                                                                                                                                           &                                                                                                                  \\ \cline{5-5} 
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           & DOP2:P2 has leadership.                                                                                          \\
                                                                                  &                                                                  &                                                                                              &                                                                                                                                                                                           &                                                                                                                  \\ \cline{5-5} 
\textbf{}                                                                         &                                                                  &                                                                                              &                                                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}NDO: Leadership is\\ indiscernible.\end{tabular}                                      \\
                                                                                  &                                                                  &                                                                                              &                                                                                                                                                                                           &                                                                                                                  \\ \hline
\end{tabular}
\label{Tab:CodeBook}
\end{table}
